Avoided crossings and dynamical tunneling close to excited-state quantum phase transitions

Using the Wherl entropy, we study the delocalization in phase-space of energy eigenstates in the vicinity of avoided crossing in the Lipkin-Meshkov-Glick model. These avoided crossing, appearing at intermediate energies in a certain parameter region of the model, originate classically from pairs of trajectories lying in different phase space regions, which contrary to the low energy regime, are not connected by the discrete parity symmetry of the model. As coupling parameters are varied, a sudden increase of the Wherl entropy is observed for eigenstates close to the critical energy of the excited-state quantum phase transition (ESQPT). This allows to detect when an avoided crossing is accompanied by a superposition of the pair of classical trajectories in the Husimi functions of eigenstates. This superposition yields an enhancement of dynamical tunneling, which is observed by considering initial Bloch states that evolve partially into the partner region of the paired classical trajectories, thus breaking the quantum-classical correspondence in the evolution of observables.

==> coverLett.tex <==
In the submitted manuscript, we present a detailed study of the avoided-crossings occurring at intermediate energy in 
a parameter region of the well-known Lipkin-Meshkov-Glick model. Because of its simplicity and also its rich properties, this model has served from a theoretical point of view, as a testing model to prove and understand diverse phenomena also present in more elaborated models. Nonetheless, it is also of interest of experimental groups because it has been possible to realize the model in several platforms. We use a phase-space  approach and semi-classical analysis  to gain insights in the avoided crossings and establish the relation between the behaviour of the Wherl entropy, superposition of classical trajectories,  related dynamical tunneling and breaking of the classical-quantum correspondence. The presented study could be of interest of groups working in several critical phenomena as  excited-state and dynamical phase transitions. Though focused on the Lipking-Meshkov-Glick model, the identified mechanism operating on it, could also  be present in other models, which broadens the potential interest of our  manuscript.  

The authors
Daniel J. Nader
Carlos A.  González-Rodríguez
Sergio Lerma-Hernández       
